A Global Analysis of Pre-Earthquake Ionospheric Anomalies

Local ionospheric density anomalies have been reported in the days prior to major earthquakes. This global study statistically investigates whether consistent ionospheric anomalies occur in the 24 hours prior to earthquakes across different regions, magnitudes, temporal and spatial scales. We match earthquake data to Total Electron Content (TEC) data from 2000-2020 at a higher resolution and cadence than previous assessed. Globally, no significant, consistent anomaly is found. Regionally, statistically significant ionospheric anomalies arise in the 12 hours prior to earthquakes with $p \leq 0.01$ following Wilcoxon tests. For the Japanese region we find a median negative ionospheric anomaly of around 0.5 TECU between 3 and 8 hours before earthquakes. For the South American region, the median TEC is enhanced by up to ~ 2 TECU, between 7 and 10 hours before an event. We show that the results are robust to different definitions of the ''local'' region and earthquake magnitude. This demonstrates the promise of monitoring the ionosphere as part of a multimodal earthquake forecasting system.

==> references.tex <==
@article{kamogawa2013ionospheric,
  title={Is an ionospheric electron enhancement preceding the 2011 Tohoku-Oki earthquake a precursor?},
  author={Kamogawa, Masashi and Kakinami, Yoshihiro},
  journal={Journal of Geophysical Research: Space Physics},
  volume={118},
  number={4},
  pages={1751--1754},
  year={2013},
  publisher={Wiley Online Library}
}

@article{xiong2021pre,
  title={Pre-Earthquake Ionospheric Perturbation Identification Using CSES Data via Transfer Learning},
  author={Xiong, Pan and Long, Cheng and Zhou, Huiyu and Battiston, Roberto and De Santis, Angelo and Ouzounov, Dimitar and Zhang, Xuemin and Shen, Xuhui},
  journal={Frontiers in Environmental Science},
  pages={514},
  year={2021},
  publisher={Frontiers}
}

@article{conti2021critical,
  title={A critical review of ground based observations of earthquake precursors},
  author={Conti, Livio and Picozza, Piergiorgio and Sotgiu, Alessandro},
  journal={Frontiers in Earth Science},
  volume={9},
  pages={676766},
  year={2021},
  publisher={Frontiers Media SA}
}

@article{moldovan2012correlation,
  title={Correlation of geomagnetic anomalies recorded at Muntele Rosu Seismic Observatory (Romania) with earthquake occurrence and solar magnetic storms},
  author={Moldovan, Iren Adelina and Placinta, Anica Otilia and Constantin, Angela Petruta and Moldovan, Adrian Septimiu and Ionescu, Constantin},
  journal={Annals of Geophysics},
  volume={55},
  number={1},
  year={2012}
}

@book{pulinets2004ionospheric,
  title={Ionospheric precursors of earthquakes},
  author={Pulinets, Sergey and Boyarchuk, Kyrill},
  year={2004},
  publisher={Springer Science \& Business Media}
}

 @article{usgs2022, title={Search Earthquake Catalog}, url={https://earthquake.usgs.gov/earthquakes/search/}, journal={Earthquake Hazards Program}, author={{USGS}}, year={2022}} 
 
 @article{sun2022matrix,
  title={Matrix completion methods for the total electron content video reconstruction},
  author={Sun, Hu and Hua, Zhijun and Ren, Jiaen and Zou, Shasha and Sun, Yuekai and Chen, Yang},
  journal={The Annals of Applied Statistics},
  volume={16},
  number={3},
  pages={1333--1358},
  year={2022},
  publisher={Institute of Mathematical Statistics}
}

 @article{cedar2022, title={Madrigal Database}, url={http://cedar.openmadrigal.org/}, author={{CEDAR}}, year={2022}} 
 
 @misc{gjerloev2022, title={SuperMAG: Global magnetic field observations}, url={https://supermag.jhuapl.edu/}, journal={SuperMAG}, author={Gjerloev, Jesper W}, year={2022}}
 
 @misc{nasa2022, title={OMNIWeb}, url={https://omniweb.gsfc.nasa.gov/ow_min.html}, journal={Space Physics Data Facility}, author={NASA}, year={2022}} 
 
 @article{cambiotti2020earthquake,
  title={On earthquake detectability by the next-generation gravity mission},
  author={Cambiotti, Gabriele and Douch, Karim and Cesare, Stefano and Haagmans, Roger and Sneeuw, Nicolas and Anselmi, Alberto and Marotta, Anna Maria and Sabadini, Roberto},
  journal={Surveys in Geophysics},
  volume={41},
  number={5},
  pages={1049--1074},
  year={2020},
  publisher={Springer}
}

 @misc{cred2021, title={EM-DAT The International Disaster Database}, url={https://www.emdat.be/index.php}, journal={EM-DAT}, author={{Centre for research on the Epidemiology of Disasters}}, year={2021}} 

 @article{Galvan2011,
author = {Galvan, David A. and Komjathy, Attila and Hickey, Michael P. and Mannucci, Anthony J.},
title = {The 2009 Samoa and 2010 Chile tsunamis as observed in the ionosphere using GPS total electron content},
journal = {Journal of Geophysical Research: Space Physics},
volume = {116},
number = {A6},
pages = {},
keywords = {ionosphere, tsunami, TEC, total electron content, gravity wave, TID},
doi = {https://doi.org/10.1029/2010JA016204},
url = {https://agupubs.onlinelibrary.wiley.com/doi/abs/10.1029/2010JA016204},
eprint = {https://agupubs.onlinelibrary.wiley.com/doi/pdf/10.1029/2010JA016204},
abstract = {Ground-based Global Positioning System (GPS) measurements of ionospheric total electron content (TEC) show variations consistent with atmospheric internal gravity waves caused by ocean tsunamis following two recent seismic events: the Samoa earthquake of 29 September 2009 and the Chile earthquake of 27 February 2010. Both earthquakes produced ocean tsunamis that were destructive to coastal communities near the epicenters, and both were observed in tidal gauge and buoy measurements throughout the Pacific Ocean. We observe fluctuations in TEC correlated in time, space, and wave properties with these tsunamis using the Jet Propulsion Laboratory's Global Ionospheric Mapping software. These TEC measurements were band-pass filtered to remove ionospheric TEC variations with wavelengths and periods outside the typical range for tsunamis. Observable variations in TEC appear correlated with the tsunamis in some locations (Hawaii and Japan), but not in others (Southern California or near the epicenters). Where variations are observed, the typical amplitude tends to be ∼0.1–0.2 TEC units for these events, on the order of ∼1\% of the background TEC value. These observations are compared to estimates of expected tsunami-driven TEC variations produced by Embry Riddle Aeronautical University's Spectral Full Wave Model, an atmosphere-ionosphere coupled model, and are found to be in good agreement. Significant TEC variations are not always seen when a tsunami is present, but in these two events the regions where a strong ocean tsunami was observed coincided with clear TEC observations, while a lack of clear TEC observations coincided with smaller sea surface height amplitudes. There exists the potential to apply these detection techniques to real-time GPS TEC data, providing estimates of tsunami speed and amplitude that may be useful for early warning systems.},
year = {2011}
}

@article{Vijayan2022,
title = {Detecting aliasing and artifact free co-seismic and tsunamigenic ionospheric perturbations using GPS},
journal = {Advances in Space Research},
volume = {69},
number = {2},
pages = {951-975},
year = {2022},
issn = {0273-1177},
doi = {https://doi.org/10.1016/j.asr.2021.10.040},
url = {https://www.sciencedirect.com/science/article/pii/S0273117721008000},
author = {M. {Sithartha Muthu Vijayan} and K. Shimna},
keywords = {Ionosphere, Ionospheric perturbations, GPS, Tsunami, Earthquake, Spatio-periodic leveling algorithm},
abstract = {Ionospheric perturbations induced by tsunamis and earthquakes can be used for tsunami early warning and remote sensing of earthquakes, provided the perturbations are characterized properly to distinguish them from the ones caused by other sources. The ionospheric perturbations are increasingly being obtained from Global Positioning System (GPS) based Total Electron Content (TEC) measurements sampled at uniform time intervals. However, the sampling is not uniform in space. The nonuniform spatial sampling along the GPS satellite tracks introduces aliasing if it is not accounted while computing the ionospheric perturbations. All the methods hitherto used to detect the co-seismic and tsunamigenic ionospheric perturbations did not account the nonuniform spatial sampling while computing these perturbations. In addition, the residual approach used to obtain the perturbations by detrending the TEC time series using high-order polynomial fit introduces artifacts. These aliasing and artifacts corrupt amplitude, Signal-to-Noise Ratio (SNR), phase, and frequency of ionospheric perturbations which are vital to distinguish the perturbations induced by tsunamis and earthquakes from the rest. We show that Spatio-Periodic Leveling Algorithm (SPLA) successfully removes such aliasing and artifacts. The efficiency of SPLA in removing the aliases and artifacts is validated under two simulated scenarios, and using GPS observations carried out during two natural disasters – the 2004 Indian Ocean tsunami and the 2015 Nepal-Gorkha earthquake. We, further, studied the severity of aliasing and artifacts on co-seismic and tsunamigenic perturbations by analyzing its characteristics employing SNR, spatiotemporal, and wavelet analyses. The results reveal that removal of aliasing and artifacts using SPLA i) increases the SNR up to ∼149% compared to the residual method and ∼39% compared to the differential method, ii) distinctly resolves signals from sharp static variations, and iii) detects 50% more co-seismic ionospheric perturbations and 25% more tsunami-induced ionospheric perturbations in the two events studied. Cross-correlation of the perturbation time series obtained using the residual method and SPLA reveals that aliasing and artifacts shift the time of occurrence by −7.64 minutes to +4.21 minutes. Further, the results show that the SPLA efficiently detects the ionospheric perturbations at low elevation angles, thereby removes the need of applying elevation cut-off and increases the area of ionospheric exploration of a GPS receiver.}
}

@article{Astafyeva2019,
author = {Astafyeva, E. and Shults, K.},
title = {Ionospheric GNSS Imagery of Seismic Source: Possibilities, Difficulties, and Challenges},
journal = {Journal of Geophysical Research: Space Physics},
volume = {124},
number = {1},
pages = {534-543},
keywords = {earthquakes, ionosphere, ionospheric seismology, seismo-ionospheric imagery, GNSS, coseismic ionospheric disturbances},
doi = {https://doi.org/10.1029/2018JA026107},
url = {https://agupubs.onlinelibrary.wiley.com/doi/abs/10.1029/2018JA026107},
eprint = {https://agupubs.onlinelibrary.wiley.com/doi/pdf/10.1029/2018JA026107},
abstract = {Abstract Up to now, the possibility to obtain images of seismic source from ionospheric Global Navigation Satellite Systems (GNSS) measurements (seismo-ionospheric imagery) has only been demonstrated for giant earthquakes with moment magnitude Mw => 9.0. In this work, we discuss difficulties and restrictions of this method, and we apply for the first time the seismo-ionospheric imagery for smaller earthquakes. The latter is done on the example of the Mw7.4 Sanriku-oki earthquake of 9 March 2011. Analysis of 1-Hz data of total electron content (TEC) shows that the first coseismic ionospheric disturbances (CID) occur ~470–480 s after the earthquake as TEC enhancement on the east-northeast from the epicenter. The location of these first CID arrivals corresponds to the location of the coseismic uplift that is known as the source of tsunamis. Our results confirm that despite several difficulties and limitations, high-rate ionospheric GNSS data can be used for determining the seismic source parameters for both giant and smaller/moderate earthquakes. In addition to these seismo-ionospheric applications, we raise several fundamental questions on CID nature and evolution, namely, one of the most challenging queries—can moderate earthquake generate shock-acoustic waves?},
year = {2019}
}

@article{Liu2009,
author = {Liu, J. Y. and Chen, Y. I. and Chen, C. H. and Liu, C. Y. and Chen, C. Y. and Nishihashi, M. and Li, J. Z. and Xia, Y. Q. and Oyama, K. I. and Hattori, K. and Lin, C. H.},
title = {Seismoionospheric GPS total electron content anomalies observed before the 12 May 2008 Mw7.9 Wenchuan earthquake},
journal = {Journal of Geophysical Research: Space Physics},
volume = {114},
number = {A4},
pages = {},
keywords = {GPS TEC, Sichuan earthquake, FORMOSAT3/COSMIC},
doi = {https://doi.org/10.1029/2008JA013698},
url = {https://agupubs.onlinelibrary.wiley.com/doi/abs/10.1029/2008JA013698},
eprint = {https://agupubs.onlinelibrary.wiley.com/doi/pdf/10.1029/2008JA013698},
abstract = {The global ionospheric map (GIM) is used to observe variations in the total electron content (TEC) of the global positioning system (GPS) associated with 35 M => 6.0 earthquakes that occurred in China during the 10-year period of 1 May 1998 to 30 April 2008. The statistical result indicates that the GPS TEC above the epicenter often pronouncedly decreases on day 3–5 before 17 M => 6.3 earthquakes. The GPS TEC of the GIM and electron density profiles probed by six microsatellites of FORMOSAT3/COSMIC (F3/C) are further employed to simultaneously observe seismoionospheric anomalies during an Mw7.9 earthquake near Wenchuan, China, on 12 May 2008. It is found that GPS TEC above the forthcoming epicenter anomalously decreases in the afternoon period of day 6–4 and in the late evening period of day 3 before the earthquake, but enhances in the afternoon of day 3 before the earthquake. The spatial distributions of the anomalous and extreme reductions and enhancements indicate that the earthquake preparation area is about 1650 km and 2850 km from the epicenter in the latitudinal and longitudinal directions, respectively. The F3/C results further show that the ionospheric F2 peak electron density, NmF2, and height, hmF2, significantly decreases approximately 40\% and descends about 50–80 km, respectively, when the GPS TEC anomalously reduces.},
year = {2009}
}


@article{Ikuta2022,
author = {Ikuta, R. and Oba, R.},
title = {How Credible Are Earthquake Predictions Based on TEC Variations?},
journal = {Journal of Geophysical Research: Space Physics},
volume = {127},
number = {3},
pages = {e2021JA030151},
keywords = {total electron content, earthquake precursor, earthquake prediction, global ionospheric map, ROC test},
doi = {https://doi.org/10.1029/2021JA030151},
url = {https://agupubs.onlinelibrary.wiley.com/doi/abs/10.1029/2021JA030151},
eprint = {https://agupubs.onlinelibrary.wiley.com/doi/pdf/10.1029/2021JA030151},
note = {e2021JA030151 2021JA030151},
abstract = {Abstract The possible relation between pre-earthquake processes and ionospheric fluctuations is widely investigated and debated. Here, we conduct a numerical experiment to examine two studies that reported preseismic anomalies in the ionospheric total electron content (TEC) and argue for the significance of their respective analyses based on statistical evaluations. The first study is that by Liu et al. (2018, https://doi.org/10.3319/tao.2018.03.11.01), who statistically investigated the relationship between 62 M => 6 earthquakes occurred in China over an 18-year period and the TEC, which was deduced from the Global Ionospheric Map. According to this study, the TEC showed anomalies with specific polarities at certain days and times that preceded the earthquakes. Earthquake alarms they defined based on these anomalies showed a good performance. We conduct this same analysis using random synthetic earthquakes and obtain results that closely match those by Liu et al. (2018, https://doi.org/10.3319/tao.2018.03.11.01), thus indicating that the good performance of the Liu et al. (2018, https://doi.org/10.3319/tao.2018.03.11.01) alarm is an artifact. The second study is that by Le et al. (2011, https://doi.org/10.1029/2010ja015781), who classified the TEC time series into anomalous and non-anomalous days based on the TEC perturbation. They found that the anomalous day rate increased as the nucleation time of the earthquakes was approached, especially for larger and shallower earthquakes. We conduct the same analysis using random synthetic earthquakes. The anomalous day rate that is comparable to their result occurs in ∼40\% of the 1,000 random trials, thereby suggesting that their result may also be an artifact.},
year = {2022}
}

@article{Liu2018,
abstract = {To verify the pre-earthquake ionospheric anomaly (PEIA), statistical analyses are implemented on the relationship between the total electron content (TEC) of global ionosphere map (GIM) and 62 M => 6.0 earthquakes in China during 1998 2015. A median-based method together with z test is employed to determine the criteria and/or characteristics of TEC anomalies related to earthquakes. It is found that the GIM TEC significantly decreases at 18:00 - 22:00 UT (universal time, post-midnight to pre-dawn) 4 - 5 days before 37 6.0 <= M {\textless} 6.5 earthquakes, at 01:00 - 04:00 UT (morning) 3 - 6 days before 18 6.5 <= M {\textless} 7.0 earthquakes, and 04:00 - 10:00 UT (pre-noon to afternoon) 3 - 5 days; but increases 08:00 - 12:00 UT (late afternoon to early evening), 18 - 20 days before 7 M => 7.0 earthquakes. The receiver operating characteristic (ROC) curve is used to compare the TEC anomaly-based method with some competitive alternatives for predicting the earthquakes under study. We found, based on possible TEC anomalies, that the observed PEIAs are significantly earthquake-related. Moreover, the results of regression analyses show that the PEIA strength is associated with the magnitude of earthquakes.},
author = {Liu, Cheng Yan and Liu, Jann Yenq and Chen, Yuh Ing and Qin, Fei and Chen, Wei Sheng and Xia, Ya Qin and Bai, Zhi Qiang},
doi = {10.3319/TAO.2018.03.11.01},
issn = {23117680},
journal = {Terrestrial, Atmospheric and Oceanic Sciences},
keywords = {Article,Number 5,Total electron content,Volume 29,Z test},
month = {oct},
number = {5},
pages = {485--498},
publisher = {Chinese Geoscience Union},
title = {{Statistical analyses on the ionospheric total electron content related to M >6.0 earthquakes in China during 1998 - 2015}},
url = {http://tao.cgu.org.tw/index.php/articles/archive/geophysics/item/1595},
volume = {29},
year = {2018}
}

@article{Rolland2011,
abstract = {We provide here a preliminary analysis of the ionospheric perturbations observed after the 11 March 2011 Tohoku Earthquake using a GPS-derived Total Electron Content (TEC) technique. Such anomalies are routinely observed after seismic events of magnitude Mw = 6 and more. Here, we use the high density and the wide coverage of the Japanese Global Positioning System (GPS) network GEONET to image the ionosphere just after the main shock. We describe ionospheric perturbations with exceptional extension in amplitude and duration. As already seen in earlier events, a first intense signal is observed about 10 minutes after the seismic rupture; the first response consists in two modes: one propagating beyond 3 km/s and the other at nearly 1 km/s. A further analysis of TEC time series of the latter mode near the source shows the typical frequencies of acoustic resonance. Beyond 400 km from the source, both the tsunami induced gravity wave and a third mode are imaged, the latter for the first time. We show that the pattern of this slow (225 m/s ± 10 m/s) and long period gravity wave (1.8 ± 0.2 mHz) is most visible in the North-West of the epicentral area. This description is corroborated by a computation of the normal modes of the solid Earth-atmosphere system. Copyright {\textcopyright} The Society of Geomagnetism and Earth, Planetary and Space Sciences (SGEPSS).},
author = {Rolland, Lucie M. and Lognonn{\'{e}}, Philippe and Astafyeva, Elvira and Kherani, E. Alam and Kobayashi, Naoki and Mann, Mich{\`{e}}le and Munekane, Hiroshi},
doi = {10.5047/EPS.2011.06.020/FIGURES/4},
file = {::},
issn = {18805981},
journal = {Earth, Planets and Space},
keywords = {Acoustic resonance,Earthquake,GPS-TEC,Ionosphere},
month = {sep},
number = {7},
pages = {853--857},
publisher = {Springer Berlin},
title = {{The resonant response of the ionosphere imaged after the 2011 off the Pacific coast of Tohoku Earthquake}},
url = {https://link.springer.com/articles/10.5047/eps.2011.06.020 https://link.springer.com/article/10.5047/eps.2011.06.020},
volume = {63},
year = {2011}
}

@article{Zhang2022,
abstract = {The Tonga volcano eruption at 04:14:45 UT on 2022-01-15 released enormous amounts of energy into the atmosphere, triggering very significant geophysical variations not only in the immediate proximity of the epicenter but also globally across the whole atmosphere. This study provides a global picture of ionospheric disturbances over an extended period for at least 4 days. We find traveling ionospheric disturbances (TIDs) radially outbound and inbound along entire Great-Circle loci at primary speeds of ∼300–350 m/s (depending on the propagation direction) and 500–1,000 km horizontal wavelength for front shocks, going around the globe for three times, passing six times over the continental US in 100 h since the eruption. TIDs following the shock fronts developed for ∼8 h with 10–30 min predominant periods in near- and far- fields. TID global propagation is consistent with the effect of Lamb waves which travel at the speed of sound. Although these oscillations are often confined to the troposphere, Lamb wave energy is known to leak into the thermosphere through channels such as atmospheric resonance at acoustic and gravity wave frequencies, carrying substantial wave amplitudes at high altitudes. Prevailing Lamb waves have been reported in the literature as atmospheric responses to the gigantic Krakatoa eruption in 1883 and other geohazards. This study provides substantial first evidence of their long-duration imprints up in the global ionosphere. This study was enabled by ionospheric measurements from 5,000+ world-wide Global Navigation Satellite System (GNSS) ground receivers, demonstrating the broad implication of the ionosphere measurement as a sensitive detector for atmospheric waves and geophysical disturbances.},
author = {Zhang, Shun Rong and Vierinen, Juha and Aa, Ercha and Goncharenko, Larisa P. and Erickson, Philip J. and Rideout, William and Coster, Anthea J. and Spicher, Andres},
doi = {10.3389/FSPAS.2022.871275/BIBTEX},
file = {:Users/andysmith/Library/Application Support/Mendeley Desktop/Downloaded/Zhang et al. - 2022 - 2022 Tonga Volcanic Eruption Induced Global Propagation of Ionospheric Disturbances via Lamb Waves.pdf:pdf},
issn = {2296987X},
journal = {Frontiers in Astronomy and Space Sciences},
keywords = {GNSS,Tonga volcano eruption,geohazard,lamb waves,traveling ionospheric disturbances},
month = {mar},
pages = {49},
publisher = {Frontiers Media S.A.},
title = {{2022 Tonga Volcanic Eruption Induced Global Propagation of Ionospheric Disturbances via Lamb Waves}},
volume = {9},
year = {2022}
}

@article{Rideout2006,
abstract = {A software package known as MIT Automated Processing of GPS (MAPGPS) has been developed to automate the processing of GPS data into global total electron density (TEC) maps. The goal of the MAPGPS software is to produce reliable TEC data automatically, although not yet in real time. Observations are used from all available GPS receivers during all geomagnetic conditions where data has been successfully collected. In this paper, the architecture of the MAPGPS software is described. Particular attention is given to the algorithms used to estimate the individual receiver biases. One of the largest sources of error in estimating TEC from GPS data is the determination of these unknown receiver biases. The MAPGPS approach to solving the receiver bias problem uses three different methods: minimum scalloping, least squares, and zero-TEC. These methods are described in detail, along with their relative performance characteristics. A brief comparison of the JPL and MAPGPS receiver biases is presented, and a possible remaining error source in the receiver bias estimation is discussed. Finally, the Madrigal database, which allows Web access to the MAPGPS TEC data and maps, is described.},
author = {Rideout, William and Coster, Anthea},
doi = {10.1007/S10291-006-0029-5/FIGURES/6},
file = {:Users/andysmith/Library/Application Support/Mendeley Desktop/Downloaded/Rideout, Coster - 2006 - Automated GPS processing for global total electron content data.pdf:pdf},
issn = {10805370},
journal = {GPS Solutions},
keywords = {Atmospheric Sciences,Automotive Engineering,Electrical Engineering,Geophysics/Geodesy,Space Exploration and Astronautics),Space Sciences (including Extraterrestrial Physics},
month = {jul},
number = {3},
pages = {219--228},
publisher = {Springer},
title = {{Automated GPS processing for global total electron content data}},
url = {https://link.springer.com/article/10.1007/s10291-006-0029-5},
volume = {10},
year = {2006}
}

@article{Thomas2017,
author = {Thomas, J. N. and Huard, J. and Masci, F.},
title = {A statistical study of global ionospheric map total electron content changes prior to occurrences of M=>6.0 earthquakes during 2000–2014},
journal = {Journal of Geophysical Research: Space Physics},
volume = {122},
number = {2},
pages = {2151-2161},
keywords = {earthquake, ionosphere, prediction, TEC},
doi = {https://doi.org/10.1002/2016JA023652},
url = {https://agupubs.onlinelibrary.wiley.com/doi/abs/10.1002/2016JA023652},
eprint = {https://agupubs.onlinelibrary.wiley.com/doi/pdf/10.1002/2016JA023652},
abstract = {Abstract There are many reports on the occurrence of anomalous changes in the ionosphere prior to large earthquakes. However, whether or not these changes are reliable precursors that could be useful for earthquake prediction is controversial within the scientific community. To test a possible statistical relationship between ionospheric disturbances and earthquakes, we compare changes in the total electron content (TEC) of the ionosphere with occurrences of 1279 M=>6.0 earthquakes globally for 2000–2014. We use TEC data from the global ionosphere map (GIM) and an earthquake list declustered for aftershocks. For each earthquake, we look for anomalous changes in GIM-TEC within 2.5° latitude and 5.0° longitude of the earthquake location (the spatial resolution of GIM-TEC). Although case studies of individual earthquakes that used short periods of data sometimes yield GIM-TEC changes that were considered possible earthquake-related phenomena, our analysis has not found any statistically significant changes prior to earthquakes when considering all 1279 earthquakes together. Thus, we have found no evidence that would suggest that monitoring changes in GIM-TEC might be useful for predicting earthquakes.},
year = {2017}
}

@article{Zhu2020,
abstract = {With the rapid development of the Global Navigation Satellite System (GNSS) and its wide applications to atmospheric science research, the global ionosphere map (GIM) total electron content (TEC) data are extensively used as a potential tool to detect ionospheric disturbances related to seismic activity and they are frequently used to statistically study the relation between the ionosphere and earthquakes (EQs). Indeed, due to the distribution of ground based GPS receivers is very sparse or absent in large areas of ocean, the GIM-TEC data over oceans are results of interpolation between stations and extrapolation in both space and time, and therefore, they are not suitable for studying the marine EQs. In this paper, based on the GIM-TEC data, a statistical investigation of ionospheric TEC variations of 15 days before and after the 276 M => 6.0 inland EQs is undertaken. After eliminating the interference of geomagnetic activities, the spatial and temporal distributions of the ionospheric TEC disturbances before and after the EQs are investigated and compared. There are no particularly distinct features in the time distribution of the ionospheric TEC disturbances before the inland EQs. However, there are some differences in the spatial distribution, and the biggest difference is precisely in the epicenter area. On the other hand, the occurrence rates of ionospheric TEC disturbances within 5 days before the EQs are overall higher than those after EQs, in addition both of them slightly increase with the earthquake magnitude. These results suggest that the anomalous variations of the GIM-TEC before the EQs might be related to the seismic activities.},
author = {Zhu, Fuying and Jiang, Yingchun},
doi = {10.1038/s41598-020-74995-w},
file = {:Users/andysmith/Library/Application Support/Mendeley Desktop/Downloaded/Zhu, Jiang - 2020 - Investigation of GIM-TEC disturbances before M => 6.0 inland earthquakes during 2003–2017.pdf:pdf},
isbn = {0123456789},
issn = {2045-2322},
journal = {Scientific Reports 2020 10:1},
keywords = {Geophysics,Natural hazards},
month = {oct},
number = {1},
pages = {1--7},
pmid = {33093593},
publisher = {Nature Publishing Group},
title = {{Investigation of GIM-TEC disturbances before M=>6.0 inland earthquakes during 2003–2017}},
url = {https://www.nature.com/articles/s41598-020-74995-w},
volume = {10},
year = {2020}
}

@article{Ulukavak2020,
abstract = {In this work, a relationship between ionospheric TEC anomalies and different earthquake magnitude groups before the main shocks was investigated. For this purpose, 2942 global earthquakes with Mw=>6 from 2000 to 2019 and possible ionospheric TEC anomalies that occurred before earthquakes were examined by considering 13 different index values of space weather conditions (geomagnetic storm indices and solar activity indices). Anomalies of ionospheric TEC changes were defined for 15-days before and 4-days after the earthquakes by using 15-days moving median method with the length of 15 days. Earthquakes were first grouped according to their magnitudes, and then negative and positive TEC anomalies in quiet days before the earthquakes were detected. These anomalies were observed as ∼5–13, ∼5-10, ∼5-15, ∼3-13, ∼7-15, ∼1 and ∼5-8 days ago for the earthquakes of 6.0 <= Mw{\textless}6.5, 6.5 <= Mw{\textless}7.0, 7.0 <= Mw{\textless}7.5, 7.5 <= Mw{\textless}8.0, 8.0 <= Mw{\textless}8.5, 8.5 <= Mw{\textless}9.0, and 9.0 <= Mw{\textless}9.5, respectively. Mean of changes in TEC anomalies of these groups is 44.2 {\%} TECU and we detected that the number of positive anomalies in each group is larger than the number of negative anomalies. Consequently, these analyses clearly show that the day-to-day changes in TEC anomalies may supply significant precursors prior to the global earthquakes (M => 6) in the short-term earthquake prediction for main shocks.},
author = {Ulukavak, Mustafa and Yal{\c{c}}ınkaya, Mualla and Kayık{\c{c}}ı, Emine Tanır and {\"{O}}zt{\"{u}}rk, Serkan and Kandemir, Raif and Karslı, Hakan},
doi = {10.1016/J.JOG.2020.101721},
file = {:Users/andysmith/Library/Application Support/Mendeley Desktop/Downloaded/Ulukavak et al. - 2020 - Analysis of ionospheric TEC anomalies for global earthquakes during 2000-2019 with respect to earthquake magn.pdf:pdf},
issn = {0264-3707},
journal = {Journal of Geodynamics},
keywords = {Earthquake magnitude,Geomagnetic storm indices,Ionospheric total electron content (TEC),Solar activity indices},
month = {apr},
pages = {101721},
publisher = {Pergamon},
title = {{Analysis of ionospheric TEC anomalies for global earthquakes during 2000-2019 with respect to earthquake magnitude (Mw=>6.0)}},
volume = {135},
year = {2020}
}

@article{Lim2019,
abstract = {Various studies have investigated the link between seismic activity and ionospheric precursory phenomena. Many of these retrospective case studies have supported the existence of pre-earthquake ionospheric anomalies by examining past earthquake events using a variety of analytical methods. Based on existing methodologies, however, the conversion of a retrospective analysis to a prospective forewarning scenario is not a straightforward process. The obstacles to its potential adoption stem mainly from assumptions made during data analysis and interpretation. In this study, several parameters pertaining to existing approaches for the detection of these ionospheric anomalies are highlighted and discussed, in particular ionosphere total electron content (TEC). A detailed examination is conducted to understand the roles that each of these parameters play in the detection process and the consequent difficulties when adopting them in a prospective analysis. These issues include accounting for variations in ionosphere characteristics owing to different measurement platforms (e.g. ground- and space-based observations) and statistical methods (e.g. standard deviation envelopes) used in detecting anomalies. Furthermore, the necessity of excluding space weather contributions in the underlying TEC fluctuations poses a challenge in determining the validity of observed ionospheric anomalies. The notion of an “earthquake preparation zone” is also evaluated in the context of the ionosphere, along with its implications in a forewarning scenario. These issues need to be addressed in current research in order to enable its possible application in earthquake forewarning.},
author = {Lim, B. J.M. and Leong, E. C.},
doi = {10.1007/S00024-018-2083-7/FIGURES/17},
issn = {14209136},
journal = {Pure and Applied Geophysics},
keywords = {Earthquakes,TEC,precursor,seismo-ionospheric anomalies,statistical analysis},
month = {jun},
number = {6},
pages = {2425--2449},
publisher = {Birkhauser Verlag AG},
title = {{Challenges in the Detection of Ionospheric Pre-Earthquake Total Electron Content Anomalies (PETA) for Earthquake Forewarning}},
url = {https://link.springer.com/article/10.1007/s00024-018-2083-7},
volume = {176},
year = {2019}
}

@article{Liu2009b,
author = {Liu, Libo and Chen, Yiding},
title = {Statistical analysis of solar activity variations of total electron content derived at Jet Propulsion Laboratory from GPS observations},
journal = {Journal of Geophysical Research: Space Physics},
volume = {114},
number = {A10},
pages = {},
keywords = {ionospheric climatology, solar activity variation, GPS TEC},
doi = {https://doi.org/10.1029/2009JA014533},
url = {https://agupubs.onlinelibrary.wiley.com/doi/abs/10.1029/2009JA014533},
eprint = {https://agupubs.onlinelibrary.wiley.com/doi/pdf/10.1029/2009JA014533},
abstract = {We analyzed the data series of the total electron content (TEC) derived at Jet Propulsion Laboratory from Global Positioning System (GPS) observations to investigate the solar activity effects of TEC on a global scale. The daily values of the solar extreme ultraviolet (EUV) fluxes in 0.1–50 nm wavelengths, 10.7 cm radio flux F10.7, and F10.7P (the average of daily F10.7 and its 81-day mean F10.7A) are adopted to represent the solar EUV variability, respectively. The EUV fluxes are measured by the Solar EUV Monitor (SEM) spectrometer aboard Solar Heliospheric Observatory (SOHO). Three kinds of patterns (linearity, saturation, and amplification) can be detected in TEC versus F10.7P and EUV. A saturation feature exists in TEC versus F10.7 in the daytime, more pronounced at low latitudes than at middle and high latitudes. The saturation in the equatorial anomaly regions is strongest in equinoxes and weakest in the June solstice. In contrast, the amplification in TEC, as a novel feature, is mainly distributed in the northern middle, and high latitudes in the December solstice and in the Southern Hemisphere in the June solstice and the March equinox. It is the first time to determine where and when the linear, saturation, and amplification patterns are distributed in TEC. Further, the solar activity sensitivity of TEC is stronger at day than at night and more evident at lower latitudes than at higher latitudes. The solar activity dependent rates of TEC in the equatorial and low-latitude regions have a minimum around the dip equator and maxima on both sides of the dip equator (near the crest of the equatorial anomaly). This structure is roughly aligned along the dip equator, being strongest in equinoxes and weakest in the June solstice, which highlights the importance of ionospheric dynamics related with E × B drift. In addition, this analysis confirms that in a statistical sense, a quadrate polynomial can well capture the long-term solar activity dependency of TEC at specified local time.},
year = {2009}
}

@article{Mendillo2006,
author = {Mendillo, Michael},
title = {Storms in the ionosphere: Patterns and processes for total electron content},
journal = {Reviews of Geophysics},
volume = {44},
number = {4},
pages = {},
keywords = {ionospheric storms},
doi = {https://doi.org/10.1029/2005RG000193},
url = {https://agupubs.onlinelibrary.wiley.com/doi/abs/10.1029/2005RG000193},
eprint = {https://agupubs.onlinelibrary.wiley.com/doi/pdf/10.1029/2005RG000193},
abstract = {The ionosphere's total electron content (TEC) is a parameter widely used in studies of the near-Earth plasma environment. The scientific use of TEC appeared early in the artificial satellite era, and among its many contributions were fundamental insights into how the ionosphere responds to geomagnetic storms. While many excellent reviews of solar-terrestrial disturbances exist in the literature, none have concentrated on the TEC parameter per se. With new TEC data sets increasingly available from the Global Positioning System (GPS), a comprehensive summary of pre-GPS storm studies is needed to set the base for progress in the GPS era. This review summarizes past case studies, describes statistical occurrence pattern, and identifies responsible mechanisms validated via modeling. It presents a new set of results of TEC disturbance patterns during 180 geomagnetic storms to describe seasonal and solar cycle effects. It concludes with a set of open questions that require additional study.},
year = {2006}
}

@inbook{Prolss2008,
author = {Prölss, Gerd W.},
publisher = {American Geophysical Union (AGU)},
isbn = {9781118666555},
title = {Ionospheric Storms at Mid-Latitude: A Short Review},
booktitle = {Midlatitude Ionospheric Dynamics and Disturbances},
chapter = {},
pages = {9-24},
doi = {https://doi.org/10.1029/181GM03},
url = {https://agupubs.onlinelibrary.wiley.com/doi/abs/10.1029/181GM03},
eprint = {https://agupubs.onlinelibrary.wiley.com/doi/pdf/10.1029/181GM03},
year = {2008},
keywords = {Ionosphere—Research, Ionospheric storms, Sudden ionospheric disturbances, Space environment},
abstract = {Summary This chapter contains sections titled: Introduction Early History of Ionospheric Storm Research Publication Statistics Defining Middle Latitudes Positive Ionospheric Storms}
}

@article{Kane2003,
title = {Solar EUV and ionospheric parameters: A brief assessment},
journal = {Advances in Space Research},
volume = {32},
number = {9},
pages = {1713-1718},
year = {2003},
issn = {0273-1177},
doi = {https://doi.org/10.1016/S0273-1177(03)90467-4},
url = {https://www.sciencedirect.com/science/article/pii/S0273117703904674},
author = {R.P. Kane},
abstract = {Percentage changes in Nm, i.e., in (foF2) should be the same as percentage changes in solar EUV. If there is a mismatch, it would be attributed to the contributions to Nm of other factors like neutral density, temperature, composition, neutral winds and electric fields, all of which vary with solar EUV. For the AE-E data of 1977–1981, the (foF2)2 values at several locations increased from 1.0 (base level for January 1978) to a peak value ratio of ∼2.0 in 1980, while the integrated flux for 18–910 \hat{A} appropriate for foF2 changes was ∼ 2.00, just enough for causing the observed foF2 changes. Thus, during 1978–1980, the contribution from other factors must be small, though for the longer interval 1976–1980, Richards [2001] reported substantial contribution from other factors. Since 1996, SEM/SOHO has made EUV measurements in the 260–340 Å range. From the solar minimum in 1996 to the solar maximum in 2000, this EUV increased by a factor of only 2.4, but the (foF2)2 at several locations have increased by a factor of 3.0 or more. Thus, in cycle 23, the contribution of other factors to Nm increase must have been substantial. In 27-day sequences of EUV, (foF2)2 did not always show similar fluctuations.}
}

@article{Hickey2009,
author = {Hickey, M. P. and Schubert, G. and Walterscheid, R. L.},
title = {Propagation of tsunami-driven gravity waves into the thermosphere and ionosphere},
journal = {Journal of Geophysical Research: Space Physics},
volume = {114},
number = {A8},
pages = {},
keywords = {tsunami, atmosphere, waves},
doi = {https://doi.org/10.1029/2009JA014105},
url = {https://agupubs.onlinelibrary.wiley.com/doi/abs/10.1029/2009JA014105},
eprint = {https://agupubs.onlinelibrary.wiley.com/doi/pdf/10.1029/2009JA014105},
abstract = {Recent observations have revealed large F-region electron density perturbations (∼100\%) and total electron content (TEC) perturbations (∼30\%) that appear to be correlated with tsunamis. The characteristic speed and horizontal wavelength of the disturbances are ∼200 m/s and ∼400 km. We describe numerical simulations using our spectral full-wave model (SFWM) of the upward propagation of a spectrum of gravity waves forced by a tsunami, and the interaction of these waves with the F-region ionosphere. The SFWM describes the propagation of linear, steady-state acoustic-gravity waves in a nonisothermal atmosphere with the inclusion of eddy and molecular diffusion of heat and momentum, ion drag, Coriolis force, and height-dependent mean winds. The tsunami is modeled as a deformation of our model lower boundary traveling at the shallow water wave speed of 200 m/s with a maximum vertical displacement of 50 cm and described by a modified Airy function in the horizontal direction. The derived vertical velocity spectrum at the surface describes the forcing at the lower boundary of the SFWM. A steady-state 1-D ionospheric perturbation model is used to calculate the electron density and TEC perturbations. The molecular diffusion strongly damps the waves in the topside (>300-km altitude) ionosphere. In spite of this, the F-region response is large, with vertical displacements of ∼2 to 5 km and electron density perturbations of ∼100\%. Mean winds have a profound effect on the ability of the waves to propagate into the F-region ionosphere.},
year = {2009}
}

@Article{Liu2004,
AUTHOR = {Liu, J. Y. and Chuo, Y. J. and Shan, S. J. and Tsai, Y. B. and Chen, Y. I. and Pulinets, S. A. and Yu, S. B.},
TITLE = {Pre-earthquake ionospheric anomalies registered by continuous GPS TEC measurements},
JOURNAL = {Annales Geophysicae},
VOLUME = {22},
YEAR = {2004},
NUMBER = {5},
PAGES = {1585--1593},
URL = {https://angeo.copernicus.org/articles/22/1585/2004/},
DOI = {10.5194/angeo-22-1585-2004}
}

@book{Conover1971,
  title={Practical Nonparametric Statistics},
  author={Conover, W.J.},
  isbn={9780471168515},
  lccn={lc74126223},
  url={https://books.google.co.uk/books?id=NV4YAAAAIAAJ},
  year={1971},
  publisher={Wiley}
}

@article{Wilcoxon1945,
 ISSN = {00994987},
 URL = {http://www.jstor.org/stable/3001968},
 author = {Frank Wilcoxon},
 journal = {Biometrics Bulletin},
 number = {6},
 pages = {80--83},
 publisher = {[International Biometric Society, Wiley]},
 title = {Individual Comparisons by Ranking Methods},
 urldate = {2023-05-10},
 volume = {1},
 year = {1945}
}

@article{freund2010toward,
  title={Toward a unified solid state theory for pre-earthquake signals},
  author={Freund, Friedemann},
  journal={Acta Geophysica},
  volume={58},
  pages={719--766},
  year={2010},
  publisher={Springer}
}

@article{kuo2011ionosphere,
  title={Ionosphere plasma bubbles and density variations induced by pre-earthquake rock currents and associated surface charges},
  author={Kuo, CL and Huba, JD and Joyce, G and Lee, LC},
  journal={Journal of Geophysical Research: Space Physics},
  volume={116},
  number={A10},
  year={2011},
  publisher={Wiley Online Library}
}

@article{sorokin2020review,
  title={A review on electrodynamic influence of atmospheric processes to the ionosphere},
  author={Sorokin, Valery M and Chmyrev, Vitaly M and Hayakawa, Masashi},
  journal={Open Journal of Earthquake Research},
  volume={9},
  number={2},
  pages={113--141},
  year={2020},
  publisher={Scientific Research Publishing}
}

@article{CEDAR_2023, url={http://cedar.openmadrigal.org/}, journal={Madrigal Database}, author={CEDAR}, year={2023}} 

@article{pulinets1998seismic,
  title={Seismic activity as a source of the ionospheric variability},
  author={Pulinets, SA},
  journal={Advances in Space Research},
  volume={22},
  number={6},
  pages={903--906},
  year={1998},
  publisher={Elsevier}
}

@article{pulinets2003main,
  title={Main phenomenological features of ionospheric precursors of strong earthquakes},
  author={Pulinets, SA and Legen'Ka, AD and Gaivoronskaya, TV and Depuev, V Kh},
  journal={journal of atmospheric and solar-terrestrial physics},
  volume={65},
  number={16-18},
  pages={1337--1347},
  year={2003},
  publisher={Elsevier}
}

@article{liu2006statistical,
  title={A statistical investigation of preearthquake ionospheric anomaly},
  author={Liu, JANN-YENQ and Chen, YI and Chuo, YJ and Chen, Chun-Shu},
  journal={Journal of Geophysical Research: Space Physics},
  volume={111},
  number={A5},
  year={2006},
  publisher={Wiley Online Library}
}

@article{le2011statistical,
  title={A statistical analysis of ionospheric anomalies before 736 M6. 0+ earthquakes during 2002--2010},
  author={Le, Huijun and Liu, Jann-Yenq and Liu, Libo},
  journal={Journal of Geophysical Research: Space Physics},
  volume={116},
  number={A2},
  year={2011},
  publisher={Wiley Online Library}
}

@article{li2013statistical,
  title={Statistical analysis of an ionospheric parameter as a base for earthquake prediction},
  author={Li, Mei and Parrot, Michel},
  journal={Journal of Geophysical Research: Space Physics},
  volume={118},
  number={6},
  pages={3731--3739},
  year={2013},
  publisher={Wiley Online Library}
}

@article{parrot2018statistical,
  title={Statistical analysis of the ionospheric density recorded by the demeter satellite during seismic activity},
  author={Parrot, Michel and Li, Mei},
  journal={Pre-earthquake processes: a multidisciplinary approach to earthquake prediction studies},
  pages={319--328},
  year={2018},
  publisher={Wiley Online Library}
}

@misc{molenkamp2023validating,
  title={Validating and comparing Total Electron Content estimates from Incoherent Scatter Radar and Global Positioning System},
  author={Molenkamp, Sven},
  year={2023}
}

@article{kelley2017apparent,
  title={Apparent ionospheric total electron content variations prior to major earthquakes due to electric fields created by tectonic stresses},
  author={Kelley, Michael C and Swartz, Wesley E and Heki, Kosuke},
  journal={Journal of Geophysical Research: Space Physics},
  volume={122},
  number={6},
  pages={6689--6695},
  year={2017},
  publisher={Wiley Online Library}
}

@article{muafiry20203,
  title={3-D tomography of the ionospheric anomalies immediately before and after the 2011 Tohoku-oki (Mw9. 0) earthquake},
  author={Muafiry, Ihsan Naufal and Heki, Kosuke},
  journal={Journal of Geophysical Research: Space Physics},
  volume={125},
  number={10},
  pages={e2020JA027993},
  year={2020},
  publisher={Wiley Online Library}
}
